MultiContrievers: Analysis of Dense Retrieval Representations

Dense retrievers compress source documents into (possibly lossy) vector representations, yet there is little analysis of what information is lost versus preserved, and how it affects downstream tasks. We conduct the first analysis of the information captured by dense retrievers compared to the language models they are based on (e.g., BERT versus Contriever). We use 25 MultiBert checkpoints as randomized initialisations to train MultiContrievers, a set of 25 contriever models. We test whether specific pieces of information -- such as gender and occupation -- can be extracted from contriever vectors of wikipedia-like documents. We measure this extractability via information theoretic probing. We then examine the relationship of extractability to performance and gender bias, as well as the sensitivity of these results to many random initialisations and data shuffles. We find that (1) contriever models have significantly increased extractability, but extractability usually correlates poorly with benchmark performance 2) gender bias is present, but is not caused by the contriever representations 3) there is high sensitivity to both random initialisation and to data shuffle, suggesting that future retrieval research should test across a wider spread of both.

==> figures/inlp_rq3.tex <==
\begin{figure}[t]
    \centering   
    \includegraphics[width=0.4\textwidth]{figures/inlp/inlp_alloc_bias.pdf}
    \caption{Causal analysis of allocational gender bias in the NQ gendered entity queries subset. Difference in performance between male (blue) and female (orange entities is allocational bias. When gender is removed from the representations via INLP, the same gap in performance remains, showing that bias is not due entirely to gender information in the representations.} 
    \label{fig:inlp_rq3}
    \vspace{-1em}
\end{figure}


==> figures/subset_correlation.tex <==
\begin{figure*}[t]
    \centering   

    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=\textwidth]{figures/correlation/NDCG@10_nq-train-new-gender-constraint_raw_scatter.pdf}
        \caption{correlation on gender subset}
        \label{fig:gender_subset_corr}
    \end{subfigure}
    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=\textwidth]{figures/correlation/NDCG@10_nq-train-new-complement_raw_scatter.pdf}
        \caption{correlation on control}
        \label{fig:control_subset_corr}
    \end{subfigure}
    \caption{tldr} 
    \label{fig:subset_performance_correlation}
    \vspace{-1em}
\end{figure*}


==> front_page.tex <==
\begin{figure}[t]
    \centering   
    \includegraphics[width=0.4\textwidth]{figures/diagrams/front_example.pdf}
    \caption{Analysis framework. Black arrows are training, dotted arrows are measurements, red fonts are metrics. We initialise and train 25 MultiContrievers from 25 MultiBerts, and measure the variance of their retrieval performance and their allocational gender bias from random variation. We also measure the variance in how well they encode gender and topic information, and how this is different from the base Bert models.} 
    \label{fig:front_example}
    \vspace{-1em}
\end{figure}

==> tables/seed_ranking.tex <==
\begin{table}[]
\resizebox{\textwidth}{!}{\begin{tabular}{llllllllllllllll}
            & arguana & climate-fever & fiqa & nf-corpus & scidocs & scifact & trec-covid & webis-touche & dbpedia-entity & fever & hotpotqa & msmarco & nq  & quora & all \\
\hline
best\_seed  & 16      & 5             & 1    & 6         & 0       & 5       & 10         & 8            & 17             & 0     & 8        & 23      & 4   & 24    & 24  \\
worst\_seed & 8       & 10            & 4    & 14        & 5       & 10      & 19         & 18           & 10             & 18    & 10       & 10      & 10  & 20    & 10  \\
\hline
delta       & 6.1     & 3.8           & 6.3  & 3.2       & 0.9     & 4.2     & 14.5       & 6.6          & 6.5            & 6.6   & 16.9     & 4       & 6.5 & 4.5   & 3.9
\end{tabular}}
\caption{Best and worst performing seeds per BEIR dataset, with delta in NDCG@10
\prcomment{Is this literally seed number? If so, I don't think this merits a table since the value of the seed itself isn't that important. Figure 1 covers the same information by showing the distribution of seed perf? If we want to have deltas, then those could be added information on top of that figure}
}
\label{tab:seed_rank}
\vspace{-1em}
\end{table}

